Understanding Entrainment in Human Groups: Optimising Human-Robot Collaboration from Lessons Learned during Human-Human Collaboration

Successful entrainment during collaboration positively affects trust, willingness to collaborate, and likeability towards collaborators. In this paper, we present a mixed-method study to investigate characteristics of successful entrainment leading to pair and group-based synchronisation. Drawing inspiration from industrial settings, we designed a fast-paced, short-cycle repetitive task. Using motion tracking, we investigated entrainment in both dyadic and triadic task completion. Furthermore, we utilise audio-video recordings and semi-structured interviews to contextualise participants' experiences. This paper contributes to the Human-Computer/Robot Interaction (HCI/HRI) literature using a human-centred approach to identify characteristics of entrainment during pair- and group-based collaboration. We present five characteristics related to successful entrainment. These are related to the occurrence of entrainment, leader-follower patterns, interpersonal communication, the importance of the point-of-assembly, and the value of acoustic feedback. Finally, we present three design considerations for future research and design on collaboration with robots.

==> Chapters/IRBMail.tex <==

\newpage
\section*{Questions: Follow-up IRB questions for protocol \#2111010723}
\begin{enumerate}
    \item Instructions that would be given to participants for the specific assembly tasks.
    \item What the collaborative tasks would be, and in what way would they interact with the robots?  Is it a physical interaction, interaction through giving robots remote direction with some sort of input, such as a keyboard, buttons, external controls, or voice commands? 
    \item How fast-paced is the assembly task-can this be explained?
    \item Can you provide some pictures/illustration of the task space and what will happen within it?  Photos or diagrams are particularly helpful.
    \item What are the specific types of “localization sensors” that will be used (brand, manufacturer), where will they be placed (i.e. on participants?) and how are they attached?
    \item Can you also send copies of the post task survey, as well as the semi-structured interview questions?
\end{enumerate}


\subsection*{(1) Task description}
Participants will be read (also provided as written material) a description of each of the two tasks. Each of the two tasks will be performed \textit{either} in pairs or in triads, and each participant only receives a description relevant for his/her condition (dyadic or triadic).

\subsubsection*{Task 1}
The first task was inspired by typical industrial assembly. For the \textit{dyadic} setting, the first participant (P1) will be lifting a bowl and hold it in front of him/her between participants. P1 would pick up the bowl and hold it in a manner that it was accessible for participant 2 (P2) to drop a small counting cube ($1\times1\times1$ cm plastic cube) in it. Following the insertion, P1 would turn around and drop the cube out of the bowl, while P2 would turn around to pick up the next cube, and the task would start again in a (potentially) infinite cycle. In the \textit{triadic} setting, the task will be identical with a minor adjustment. Here participant 3 (P3) would mimic P2 task of dropping cube in the bowl, it is up to all two/three of them to negotiate (explicitly or implicitly) the point-of-assembly in a manner that allows all P1/P2/P3 optimal access to the bowl.


\subsubsection*{Task 2}
The second task is a simple envelope stamping task. In the \textit{dyadic} setting, P1 is seated between two differently coloured stacks of envelopes (red and blue). P2 is sitting opposite P1 with two differently coloured stamps (red and blue). The tasks required P1 and P2 to stamp the letters with the corresponding stamps (red letter/red stamp, blue letter/blue stamp). P1 would take one letter at a time---of any of the two stacks---and place it between P1 and P2. P2 would, after identifying what colour P1 picked up, select the appropriate stamp and stamp the letter on the front, after which P1 would remove it, and the cycle would start again. For the \textit{triadic} setting a minor addition was made. Here P3 would place a shipping label on the letter, on which P2 would place the stamp of the corresponding colour.\\

For both tasks and both settings (dyadic and triadic), successful completion of the tasks required all participants to `bring' their respective item (Task 1: bowl, cube; Task 2: envelope, shipping label, stamp) to the same spatial position at the same time---thereby achieving both temporal and spatial synchronisation. Furthermore, the roles (P1, P2 or P3) were negotiated (explicitly and implicitly) by participants themselves without further instructions. The same goes for the point-of-assembly (p-o-a).



\subsection*{(2) Interaction with the robot}
A description of the task can be seen above (1). Participants will never need to touch the robot or vice-versa. Both participants and robot will move towards the same space in order to drop the cube (task 1) or place the envelope/shipping label (task 2). 

\subsection*{(3) Task speed}
The movement speed is human defined, meaning the tasks will be completed at a speed (chosen by participants) at which they feel comfortable. For experiments involving the robot, human will again set the pace. That is, humans will move at a comfortable space, and the robot will match the speed. 

\subsection*{(4) Illustration of task space}
To give a better overview of the space in which the experiment will be conducted, we attached an illustration of the area, see Figure~\ref{fig:area} in the Appendix. The robot in the triadic human condition will be replace with a third participant. 


\newpage
\subsection*{(5) Sensors used for localisation}

We are utilising the Optitrack Motion Tracking System to perform localisation. The OptiTrack system uses a eighteen cameras to track points of interest. Specifically, each human participant will were gloves (OptiTrack Hand Glove) that have markers (Rigid Bodies Marker Sets) attached to the back of the hand using velcro. The OptiTrack system will use these markers to calculate the location of the left and right hand of each participant.\\

\noindent
Links to equipment:
\begin{enumerate}
    \item[i.] Cameras: \url{https://optitrack.com/cameras/flex-13/}
    \item[ii.] Mocap Gloves: \url{https://optitrack.com/accessories/wear/}
    \item [iii.]Hand Rigid Bodies Marker Set: \url{https://optitrack.com/accessories/markers/#mcp1230}
\end{enumerate}

\subsection*{(6) Topics for post task survey and interview}
As the \textit{exact} questions for the interview and questionnaire are still under development, we will provide broader (\textit{fixed}) topics for these.\\

\noindent
The questionnaire will include data on i) demographics (e.g., age, gender, or prior robot experience), ii) familiarity with other participants in dyad/triad in the group (e.g., friend, family, acquaintance, stranger, etc.), iii) Big Five to identify the participants agreeableness and extraversion trait as these are directly related to better cooperation capabilities (as used by similar research~\cite{Beersma:2003,Roy:2020}).\\

\noindent
The interview will be structured around i) general experience during the task, ii) preferences towards what role (P1/P2/P3) each individual would prefer, iii) experiences in explicit and implicit negotiation of point-of-handover, iv) trust towards other participants/robot, v) perceived performance at task completion, and vi) perception of performance increase or decrease.







\bibliographystyle{ACM-Reference-Format}
\bibliography{biblio}


\vspace{2cm}
\section*{Appendix}
\begin{figure}[h]
    \centering
    \includegraphics[width=0.7\textwidth]{Figures/experiment.png}
    \captionsetup{width=.7\textwidth}
    \caption{Illustration of experimental area. Both the experiment---both tasks in both conditions---as well as the interviews and questionnaire will be performed in this area.}
    \label{fig:area}
\end{figure}



==> Chapters/Results_OLDNOTES.tex <==





-----
The optimal point of assembly is equal distance from every collaborator.


\begin{quote}
    \textit{`I try. I think I initially tried to get them as central as possible. Okay. And then I gradually decrease my own range of motion basically.'} - G6 T2 Stamp\\
\end{quote}

The placement of the point of assembly is tuned towards the bowler/enveloper.
\begin{quote}
    \textit{`I agree I was more to the side, but I wouldn't say it was like too far. It's still okay. But it was not the same as with the envelope, which was very focused on being very centrally placed. This might have been inclined towards the bin side, in this case, the bowlers left side.'} - G5 T2 Cube\\
\end{quote}

\begin{quote}
    \textit{`Because I thought it would be the easiest if I put it exactly where my hand was extended and could just turn it.'} - G7 T2 Cube\\
\end{quote}

\hl{We adjust our own behaviour as well as the point of assembly} throughout the course of the interaction. It is more important to adjust own behaviour for increase in overall team efficency rather than just optimising for our own sub-task.
\begin{quote}
    \textit{`I also noticed that like, towards the second half, both of us moved closer, or we moved our materials closer because the envelopes are being placed here.'} - G7 T1 Stamp\\
\end{quote}

\begin{quote}
    \textit{`That makes sense. [...] I also optimise for the location of the bowl, and then we can move it further down, I would rather put it there because on a global sense, that would be the best strategy considering both of your [the cubers] arms and my movement from here.'} - G2 t2 Cube\\
\end{quote}

\begin{quote}
    \textit{`I think at the end, I pushed the envelope more towards her [the stamper] because I could see like it was kind of harder. But I didn't really have like I couldn't help her in any aspect. Yeah. So yeah, that was like the only thing'.} - G8 T2 Stamp
\end{quote}
-----








\subsection{Consistency and predictability}
We make ourselves consistent and predictable. If everyone does this an optimal rhythm can be achieved.
\begin{quote}
    \textit{`I think it just gets better through iterations has, were like, each of us is like a small system or trying to optimise our behaviour. Yeah, by the same time, the relationship between us and like trying to finish our own task kind of, also, like get optimal, it's because we kind of not only try, like, we kind of become consistent not only our own behaviour, but with our expectations on other people's behaviour.'} - G1 T2 Stamp\\
\end{quote}












\subsection{Can we say something about unique differences between dyads and triads?}



\_\_\_\_\_\_\_\_\_\_\_\_\_\_\_\_\_\_\_\_\_\_\_\_\_\_\_\_\_\_\_\_\_\_\_\_\_\_\_\_\_\_\_\_\_\_\_\_\_\_\_\_
\subsection{Negotiation of the point of assembly}


List of themes that cold make (\hl{yellow} theme names are 99\%) it into the paper: 
\begin{enumerate}
    \item Synchronisation/Group rhythm: This will simply confirm that entrainment happens in team collaboration (dyads and triads) \textit{and} that this is perceived by participants.
    \item \hl{Negotiation of the point of assembly (p.o.a.):} The point of assembly is typical base-lined on minimising the variance of travel distance between all collaborators. This is, with each task iteration, optimised to account for a `temporal centre' instead of a spatial centre. Meaning, if one of the sub-tasks takes more time, the p.o.a. will be closer to this position to compensate for the temporal delay.
    \item The importance of consistency: Regardless of where the p.o.a. is placed, the most important thing is predictability and consistency.
    \item \hl{The importance of sensory information:}
\end{enumerate}


\begin{comment}
    \subsubsection{Synchronisation}
    First theme to argue that a) entrainment happens in teams, and b) that this can be either conscious or unconscious.\\
    
    \noindent
    \hl{The robot should be able to adjust its behaviour without the need for explicit telling it. This should be a permanently ongoing and organic change in rhythm.}
    
    \noindent
    When a rhythm is reached the collaboration can go into autopilot mode.
    \begin{quote}
        \textit{`I mean, we did sort of get stuck in a rhythm where we didn't really like necessarily see a lot of reason to like change what we were doing.'} - G6 T1 Cube\\
    \end{quote}
    
    \begin{quote}
        \textit{`And then like, in the beginning, we're trying to coordinate and it kind of like, reaches towards some sort of synchronisation that we don't have to pay extra attention as long as everyone's in the same tempo'} - G1 T1 Cube\\
    \end{quote}
    
    \begin{quote}
        \textit{`I think like once we got in the rhythm of Yeah. Then we were able to kind of just keep going.'} - G5 T2 Cube\\
    \end{quote}
    
    We make ourselves consistent and predictable. If everyone does this an optimal rhythm can be achieved.
    \begin{quote}
        \textit{`I think it just gets better through iterations has, were like, each of us is like a small system or trying to optimise our behaviour. Yeah, by the same time, the relationship between us and like trying to finish our own task kind of, also, like get optimal, it's because we kind of not only try, like, we kind of become consistent not only our own behaviour, but with our expectations on other people's behaviour.'} - G1 T2 Stamp\\
    \end{quote}
    
    \begin{quote}
        \textit{`Okay. So, yeah, and then finding new ways to do the task, we felt we were increasing efficiency.'} - G3 T1 Cube\\
    \end{quote}
\end{comment}

\begin{comment}
    \subsubsection{Point of assembly}
    This theme argues for the intention of the bowler/enveloper to place the bowl/envelope \textit{not just} in a way that is as easy as possible, but place it in a way that is the perfect trade-off for the entire team.\\
    
    \hl{If flexibility for the exact point of assembly is possible, this still requires consistency}
    
    \noindent
    The optimal point of assembly is equal distance from every collaborator.
    \begin{quote}
        \textit{`They were putting the cubes down at the same time. So I just need to place it in the middle.'} - G4 T1 Cube\\
    \end{quote}
    
    \begin{quote}
        \textit{`I try. I think I initially tried to get them as central as possible. Okay. And then I gradually decrease my own range of motion basically.'} - G6 T2 Stamp\\
    \end{quote}
    
    The placement of the point of assembly is tuned towards the bowler/enveloper.
    \begin{quote}
        \textit{`I agree I was more to the side, but I wouldn't say it was like too far. It's still okay. But it was not the same as with the envelope, which was very focused on being very centrally placed. This might have been inclined towards the bin side, in this case, the bowlers left side.'} - G5 T2 Cube\\
    \end{quote}
    
    \begin{quote}
        \textit{`Because I thought it would be the easiest if I put it exactly where my hand was extended and could just turn it.'} - G7 T2 Cube\\
    \end{quote}
    
    \hl{We adjust our own behaviour as well as the point of assembly} throughout the course of the interaction. It is more important to adjust own behaviour for increase in overall team efficency rather than just optimising for our own sub-task.
    \begin{quote}
        \textit{`I also noticed that like, towards the second half, both of us moved closer, or we moved our materials closer because the envelopes are being placed here.'} - G7 T1 Stamp\\
    \end{quote}
    
    \begin{quote}
        \textit{`That makes sense. [...] I also optimise for the location of the bowl, and then we can move it further down, I would rather put it there because on a global sense, that would be the best strategy considering both of your [the cubers] arms and my movement from here.'} - G2 t2 Cube\\
    \end{quote}
    
    \begin{quote}
        \textit{`I think at the end, I pushed the envelope more towards her [the stamper] because I could see like it was kind of harder. But I didn't really have like I couldn't help her in any aspect. Yeah. So yeah, that was like the only thing'.} - G8 T2 Stamp
    \end{quote}
\end{comment}

\subsubsection{Consistency is Key}
Human collaborators want consistency - but consistency does not need to be consistent. If changes are made these need to be so subtle that they are still perceived as consistent.\\

\noindent
\hl{While consistency is key - it is just as important that adjustments are made in a consistent manner.}

\begin{quote}
    \textit{`And just move in, move in and like - waste a lot less effort and have that consistently there. Yeah, I think that these two are so much dependent on the placement of the envelope.'} - G6 T2 Stamp\\
\end{quote}

\begin{quote}
    \textit{`I try, I think I initially tried to get them as central as possible, and then I gradually decrease my own range of motion basically.'} - G6 T2 Stamp\\
\end{quote}

\begin{quote}
    \textit{`So, it was like we had initially decided something we mostly kept on to it.'} - G2 T2 Cube\\
\end{quote}

\begin{quote}
    \textit{`Yeah, I think it like in theory, we all should be able to have like a consistent rhythm with it. Bring up the rhythm again.'}. - G6 T2 Stamp\\
\end{quote}





\subsubsection{Adapt pace to match group rhythm}
This section shows that individual participants adapted their pace to match the groups rhythm if they felt like they were going to slow/fast.\\

\noindent
\hl{Robots need to be able to identify who is giving the pace, based on which they need to be able to adjust.}

Example of slowing down to match the pace of collaborators.
\begin{quote}
    \textit{`I think I kind of adjusted to their speed. Because I feel like at first I think I was going too fast.'} - G8 T1 Cube\\
\end{quote}

Example of speeding up to match the pace of collaborators.
\begin{quote}
    \textit{`I thought so too. And then when I was quicker, you will also get quicker and I thought you were giving the pace and I was gonna catch up.'} - G4 T2 Stamp\\
\end{quote}


It is not always clear which collaborator sets the pace.
\begin{quote}
    \textit{`I thought so too. And then when I was quicker, you will also get quicker and I thought you were giving the pace and I was gonna catch up.'} - G4 T2 Stamp\\
\end{quote}

\subsubsection{Leader-follower pattern}
A leader follower pattern may arise, this can be related to the individual task.\\

\noindent
\hl{Depending on the task performed by the human(s) and robot(s), it is important that the robot(s) can take both roles.}
\begin{quote}
    \textit{`[Enveloper is leader] Because we depended on her. Yeah, we can only go as fast as the envelopes, which is me.'} - G7 T1 Stamp\\
\end{quote}


What is a leader? There is no leader but someone you follow.
\begin{quote}
    \textit{`I don't think there is a leader role, but I kind of follow her because I think she put the clip in first, and then I will follow.'} - G8 T1 Cube\\
\end{quote}


Multiple people can be leaders in a group based interaction.
\begin{quote}
    \textit{`I kind of just, like waited after both of them put in.'} - G8 T1 Cube
\end{quote}


\subsubsection{Second task is harder} This is not a theme but an interesting observation.


\subsubsection{Different sensory input for task completion}
Participants reported on the need to utilise multiple senses. Both \texttt{Tactile, Auditory} and \texttt{Vision} are used to synchronise motion and reach a rhythm within the group.

Sounds emitted by the task (or artificially added) can provide value when for synchronising on other interactants.

\begin{quote}
    \textit{`And then like, you know, I would work on that pretty much as much time as I had until like, I heard the stamp signal, and then I'd be like, Ah, I need to move this.'} - G10 T1 Stamp\\
\end{quote}

\begin{quote}
    \textit{`But also in this case, because I personally see like the dropping of the cube as like, a cue, like audio cue.'} - G1 T1 Cube\\
\end{quote}

\begin{quote}
    \textit{`I guess also, like auditory. Yeah, listening. Yes. Because I would like look, but I also like, make sure like, I heard something.'} - G8 T1 Cube\\
\end{quote}

\begin{quote}
    \textit{`Sound. Definitely I think, whether I knew it or not, I think I was cue'ing into that sound of ``dum dum'' [Sound of the cubes dropping in the bowl].'} - G5 T2 Cube\\
\end{quote}




\subsubsection{Robot should adapt to us}
\begin{quote}
    \textit{´I would say, Yeah, I would say if it had, if it's a robot, it should also adapt to us.'} - G4 T1 Cube\\
\end{quote}


\subsection{Motion Tracking}

\begin{enumerate}
    \item Distance between participant hands 
    \item Recovering interval time
    \item \hl{@Stan, how difficult is it to give a count based on the motion tracking for how many interactions + time stamp of each task for each group are performed? Each cycle in the signal (up-down) should represent one iteration right?}
\end{enumerate}

==> Chapters/Study_OLD.tex <==
%\section{Temporal Contingency Framework}\label{sec:ContingencyFramework}
%\hl{\textit{We should potentially have a section describing the contingency framework which forms the basis for the definition of the tasks. I'm considering to have this as one of the first subsection of the methodology section as it is strongly related to the development and selection of the two tasks.}}


\section{Methodology}\label{sec:Method}

%\subsection{Items needed}
%\begin{enumerate}
%    \item[] Assembly Task:
%    \item a light plastic bowl \\ (e.g., \url{https://www.target.com/p/37oz-plastic-cereal-bowl-navy-room-essentials-8482/-/A-82325913})
%    \item cube - could be counting cubes \\ (e.g., \url{https://www.target.com/p/learning-resources-centimeter-cubes-set-of-500-ages-6/-/A-80395819#lnk=sametab})
%    \item[]
%    \item[] Stamping Task:
%    \item 2 stamps + ink (red/blue) (Check Cornell Store)
%    \item ``Shipping labels'' \\ (e.g., \url{https://www.target.com/p/128ct-1-34-x2-75-34-rectangular-labels-white-up-38-up-8482/-/A-14471285})
%    \item Envelops \\ (\url{https://www.target.com/p/jam-paper-50pk-brite-hue-a7-envelopes-5-25-x-7-25/-/A-51376206?preselect=51216066#lnk=sametab})
%\end{enumerate}

\subsection{Participants}
We recruited X participants (\hl{demographics}). Participants where recruited using social media postings as well as flyers on campus, and consisted primarily of students from \texttt{Anonymised University} who where compensated with course credits or 15\$ pr. hour. We matched participants into dyads and triads (\hl{X dyads, Y triads}) while ensuring that they did not know (or just by face) their respective collaborators. We emphasised matching strangers, as we were interested in the identification of initial cues used to entrain during task completion. 


\subsection{Tasks}\label{sec:Tasks}
In order to investigate the research questions presented (see~\Cref{sec:Introduction}) we developed two tasks which can be investigated in both dyadic and triadic configurations. Each of these tasks was investigated in a dyadic (P1/P2) as well as triadic (P1/P2/P3) scenario, both described below. Both short-cycle repetitive tasks described, can be continued in an infinite loop - provided materials (e.g., letters or cubes) were sufficient.

\subsubsection{Task development}
In order to identify the tasks, we brainstormed potential ideas, resulting in a total of eight different tasks. Of these we prototyped seven
%tower stacking, domino, domino along line, stamp, bowl, pearl sorting, burger
which helped us define specific constraints important for the tasks. %to the identification of entrainment in human pairs/groups. 
Furthermore, the selection of tasks was inspired by~\citep[section 4.1]{Rinott:2021}. Given our eight different tasks, we plotted these along a contingency framework (see~\ref{fig:contFramework}). In order to achieve initial learnings that can be transfered to a robot, the two tasks chosen where characterised by the same pattern, i.e., `In phase'. 


\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{Figures/contFrameworkDummy.jpg}
    \caption{Dummy placeholder for the contingency framework}
    \label{fig:contFramework}
\end{figure}

%\hl{I think this section should include the description of the contingency framework} (\Cref{sec:ContingencyFramework})

%\hl{Describe clear rules of engagement for each task!}

%\hl{Describe the process of developing and deciding on these specific tasks. Including pilot-testing alternatives and reasons for these. Reasons include: easily extendable from dyads to triads, contingency (i.e., accepted delay is low - participants have to be in the same location at the same time to be able to complete the task), etc...}

\subsubsection{Task 1: Assembly task}\label{sec:Task_1}
%\hl{Note: Can this be even more simplified for the robot? Move Bowl -> put something in -> repeat}
The first task was inspired by typical industrial assembly. For the assembly task, using a robot might be beneficial, as it allows the repetitive lifting of potentially heavy materials to be performed by the robot, while lighter tasks---requiring human judgement---still would be performed by human workers.

For the \textit{dyadic} setting, P1 was responsible for lifting a bowl in between the participants. P1 would pick up the bowl and hold it in a manner that it was accessible for P2 to drop a small counting cube (cube) in it. Following the insertion, P1 would turn around and drop the cube out of the bowl, while P2 would turn around to pick up the next cube, and the task would start again in a (potentially) infinite cycle. In the \textit{triadic} setting, the task was identical with a minor adjustment. Here P3 would mimic P2 task of dropping cube in the bowl, it was now up to all three of them to negotiate the point-of-assembly in a manner that allows all both P2/P3 optimal access to the bowl

In both settings (dyadic and triadic), successful completion of the tasks required all participants to `bring' their respective item (bowl, cube, and cube) to the same spatial position at the same time---thereby achieving both temporal and spatial synchronisation. Furthermore, the roles (P1, P2 or P3) were negotiated by participants themselves without further instructions. The same goes for the point-of-assembly (p-o-a).

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{Figures/Illustration.png}
    \caption{Dummy placeholder image illustrating the first task (assembly) in the dyadic setting.}
    \label{fig:my_label}
\end{figure}


\subsubsection{Task 2: Envelope stamping}\label{sec:Task_2}
The second task was a simple envelope stamping task. In the \textit{dyadic} setting, P1 was seated between two differently coloured stacks of envelopes (red and blue). P2 was sitting opposite P1 with two differently coloured stamps (red and blue). The tasks required P1 and P2 to stamp the letters with the corresponding stamps (red letter - red stamp, blue letter - blue stamp). P1 would take one letter at a time---of any of the two stacks--- and place it between P1 and P2 while holding it in place. P2 would, after identifying what colour P1 picked up, select the appropriate stamp and stamp the letter on the front, after which P1 would remove it, and the cycle would start again. For the \textit{triadic} setting a minor addition was made. Here P3 would place a post-it note---simulating a shipping label---on the letter, on which P2 would place the stamp of the corresponding colour. 

Just as for the assembly task (see~\Cref{sec:Task_1}), the successful completion of both the dyadic and the triadic tasks requires all participants to have spatial and temporal synchronicity at the point of stamping. Again, the roles and the p-o-a were negotiated by the participants without further instructions. 


\hl{\textit{Note: Should we here enforce the need to switch between red/blue? Otherwise I fear that P2 never puts the stamp down and just hovers with stamp over the letter position. This could also be enforced by making it mandatory to put the stamp into ink after each stamp.}}

\begin{comment}
    \subsubsection{Task 3: Pattern placing}
    ``Player'' place domino bricks a long a drawn line on the table - no one is allowed to place more than one brick at anytime.
    
    This can always be extended with requirements to pattern (e.g., R-G-B-R-G-B...)
    
    \subsubsection{Task 4: "Reverse Jenga" inspired (see sketches)}
    \subsubsection{Task 5: Stamping task}
    Two stamps, stamp-ink-stamp-ink etc.
    two piles of paper
    person picks paper, robot anticipates the right stamp to use to stamp
    
    \subsubsection{Task 6: Packing task}
    human puts stuff on table, max x items on table, robots need to put stuff away to keep it under x items
    
    \subsubsection{Task 7: Colour Sorting with Counting Cubes}
    
    
    \subsubsection{Task 8: Burger Assembly}
    The task we asked participants to complete was an simple assembly task. More specifically, we asked participants to assemble as many `Styrofoam burgers' as possible within the 15 minutes allocated. Each burger consisted of \hl{X elements} simulating the bottom-bun, patty, cheese, and top-bun (see~\Cref{fig:completedBurger}. In order to enforce the need for ongoing collaboration during the assembly task we imposed to strict constraints to the task completion; a) No one person can perform all activities involved in the assembly of any given burger, and b) At no point in time can more than one `ingredient' be placed at the same time. By enforcing these two rules, we made sure that participants had to solve the assembly task in collaboration.
    
    The task was to simulate a selection of typical collaborative elements into one task with an easily comprehensible context. The burger assembly tasks involves elements such as, `pick-and-placing', interacting in a shared area, structuring collaborative work processes to mention a few. Simultaneously the assembly of a burger is a task that is easily understandable, compared to classical industrial assembly tasks.
\end{comment}

%\subsection{Data collection \& measurements}
%To collect both qualitative and quantitiave measurements, we utilised a variety of different methods for data collection. 

%\subsubsection{Quantiative data collection}
%We used the OptiTrack 


\subsection{Procedure}
%\hl{\textit{I'm thinking a within subject experiment. So we recruit e.g. 50 people and pair them into 10 dyads and 10 triads. Each dyad performs both dyadic tasks and each triad performs both triadic tasks.}}

Upon arrival in the lab participants will receive information about the study, including a description and demonstration of the two tasks (only either the dyadic or triadic version depending on the participants condition)%~\footnote{We did not demonstrate it as we tried to avoid showing them \textit{how} they were supposed to complete the task.}
, as well as information about the duration of the study. Following this, participants got the opportunity to ask questions after which the informed consent was signed.

When all questions where answered, we allowed participants a familiarisation phase with the materials of the tasks, during which researchers still were available for additional questions that might arise. Participants where asked to complete as many iterations of the task as possible within an undisclosed amount of time (inspired by~\cite{Roy:2020}). Furthermore, we emphasised that his was \textit{not} a competition between the two/three participants but that both tasks could only be completed in collaboration as individual sub-tasks dependent on one another. This was followed with a recap of the first task description and completion of the first task\footnote{Tasks order was randomised to account for ordering effects.}.

Following the task completion of the first tasks, the researcher would enter the lab setting for a short post-task interview. This was followed by a short recap of the description of the second task as well as it's completion. 

Following the second task another short post-task interview was held. Additionally, we asked participants to complete a questionnaire for the identification of participants agreeableness trait.

%Participants were instructed to assemble as many `burgers' as possible during the time frame of 15 minutes. During this time, the researchers would observe the task completion through a audio/video stream from an adjacent room. Lastly, we conducted a post-session group interview as well as debriefing in case any questions arose during the study.

\subsection{Data Collection and Analysis}
%Data Collection
In order to collect both qualitative and quantitative data we conducted the study in a usability lab equipped with an OptiTrack motion tracking system (18 cameras) to track participants hands. Additionally to the position tracking of participants hands, \hl{X} video cameras where placed to ensure audio-video recordings of participants for later identification of gaze, gesture and verbal communication. Furthermore, the video was used to extract metrics such as `Tasks completed for each 10 second interval', `Means of communication (verbal, body language, gaze)', as well as `Negotiation of roles and p-o-a'. Each task was followed by a group interview about participants experiences. The interviews were conducted in the pairs/triads to foster insightful conversation about the experience. Interviews where structured around five topics: i) participants general experience with the task, ii) preferences towards role assignment they chose, iii) experiences during the negotiation of point-of-handover, iv) trust in other participants and their capabilities to perform the task, as well as v) their perceived change (improvement, unchanged, or deterioration) in task performance.

In addition to the post-session group interview, participants filled out a questionnaire following the second task. The questionnaire included three sections including: i) demographics, ii) familiarity with other participants in the group, as well as iii) the big five personality test. The big five was added in order to identify the participants agreeableness and extraversion trait as these are directly related to better cooperation capabilities~\cite{Beersma:2003}.


%Finally, we conducted semi-structured post-session interviews with each triads in order to make them verbalise on how they attempted to achieve optimal assembly behaviour, hopefully striving towards interaction synchronicity.

%Data Analysis
As we collected a wide variety of different data streams, both qualitative and quantitative, we used a variety of data analyses methods. We coded \hl{X} interaction between members of each dyad/triad. Each interaction was clustered according to a variety of metrics such as duration, modality (e.g., gaze, speech, or gesture) as well as effect of the interaction. Furthermore, we quantified improvements in task completion in order to identify metrics used for quantification of achieved entrainment. For example, we counted amounts of assembly tasks completed during each 10-second interval, this helped us identify changes in task performance. The semi-structured post session interviews were coded to identify themes of relevance to entrainment.


\hl{Qualitative coding of Proxemics, Kinesics, and Gaze will be performed in accordance with Jinni A. Harrigan\footnote{\url{https://www.google.com/books/edition/New_Handbook_of_Methods_in_Nonverbal_Beh/YcYhlGuVnOgC?hl=en&gbpv=1&bsq=137}}}

\subsection{Measures}
Some thoughts of measures (both qual. \& quant.) that can be considered. \textit{I would like this study to utilise a mixed method approach!}

\hl{Maybe this:} Should we measure `Agreeableness' following the study? (see implication 6 in ~\cite{Roy:2020})

\hl{This:} Amount of tasks completions in each 10sec interval - i.e., how many assemblys from 1-10, 11-20, 21-30... in line with Roy and Edan~\cite{Roy:2020}. This data can easily be manually extracted from the video analysis.

\hl{This:} Extract means of communication - verbal (count or measurement?), body language, gaze~\cite{Roy:2020}

\hl{This:} Post session interview, how did they decide on point-of-handover (p-o-h) for task completion. `Where' is the assembly completed? `Where' is the paper placed on the table for stamping?

\hl{This:} Did they feel they adapted consciously to one another?

\hl{This:} Utilise passive markers for body tracking etc. (Stan knows stuff about this?)


Can we utilise some questionnaire to investigate e.g. team member agreeableness or some other metric that might tell us something?

We should (post task survey) ask how well participants know each other, post session likeability of other participants?


\hl{@Eike} Start thinking about a interview guide to inquire about information related to behaviour and why we observe what we observe. Can we see a correlation between personality trait \textit{X} and behaviour \textit{Y}? Based on the hypothesis: People with higher agreeableness perform better in cooperative tasks.

%\hl{Do we see an improvement from burger/min in minute 1 to burger/min in minute 10? This would indicate a) familiarity with the task (which is anticipated) and/or indications of a optimisation of task solving approach.}

